Centrality dependence of the pseudorapidity density distribution for charged particles in Pb-Pb collisions at $\sqrt{s_{\rm NN}}=5.02$ TeV

We present the charged-particle pseudorapidity density in Pb-Pb collisions at $\sqrt{s_{\mathrm{NN}}}=5.02\,\mathrm{Te\kern-.25exV}$ in centrality classes measured by ALICE. The measurement covers a wide pseudorapidity range from $-3.5$ to $5$, which is sufficient for reliable estimates of the total number of charged particles produced in the collisions. For the most central (0-5%) collisions we find $21\,400\pm 1\,300$ while for the most peripheral (80-90%) we find $230\pm 38$. This corresponds to an increase of $(27\pm4)\%$ over the results at $\sqrt{s_{\mathrm{NN}}}=2.76\,\mathrm{Te\kern-.25exV}$ previously reported by ALICE. The energy dependence of the total number of charged particles produced in heavy-ion collisions is found to obey a modified power-law like behaviour. The charged-particle pseudorapidity density of the most central collisions is compared to model calculations --- none of which fully describes the measured distribution. We also present an estimate of the rapidity density of charged particles. The width of that distribution is found to exhibit a remarkable proportionality to the beam rapidity, independent of the collision energy from the top SPS to LHC energies.

==> texs/acknowledgements.tex <==
% $Id: acknowledgements.tex 2270 2015-09-14 12:11:37Z loizides $
% Version: Jan 2015

The ALICE Collaboration would like to thank all its engineers and technicians for their invaluable contributions to the construction of the experiment and the CERN accelerator teams for the outstanding performance of the LHC complex.
%
The ALICE Collaboration gratefully acknowledges the resources and support provided by all Grid centres and the Worldwide LHC Computing Grid (WLCG) collaboration.
%
The ALICE Collaboration acknowledges the following funding agencies for their support in building and
running the ALICE detector:
%
State Committee of Science,  World Federation of Scientists (WFS)
and Swiss Fonds Kidagan, Armenia;
%
Conselho Nacional de Desenvolvimento Cient\'{\i}fico e Tecnol\'{o}gico (CNPq), Financiadora de Estudos e Projetos (FINEP),
Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado de S\~{a}o Paulo (FAPESP);
%
National Natural Science Foundation of China (NSFC), the Chinese Ministry of Education (CMOE)
and the Ministry of Science and Technology of China (MSTC);
%
Ministry of Education and Youth of the Czech Republic;
%
Danish Natural Science Research Council, the Carlsberg Foundation and the Danish National Research Foundation;
%
The European Research Council under the European Community's Seventh Framework Programme;
%
Helsinki Institute of Physics and the Academy of Finland;
%
French CNRS-IN2P3, the `Region Pays de Loire', `Region Alsace', `Region Auvergne' and CEA, France;
%
German Bundesministerium fur Bildung, Wissenschaft, Forschung und Technologie (BMBF) and the Helmholtz Association;
%
General Secretariat for Research and Technology, Ministry of Development, Greece;
%
Hungarian Orszagos Tudomanyos Kutatasi Alappgrammok (OTKA) and National Office for Research and Technology (NKTH);
%
Department of Atomic Energy and Department of Science and Technology of the Government of India;
%
Istituto Nazionale di Fisica Nucleare (INFN) and Centro Fermi -
Museo Storico della Fisica e Centro Studi e Ricerche ``Enrico Fermi'', Italy;
%
MEXT Grant-in-Aid for Specially Promoted Research, Ja\-pan;
%
Joint Institute for Nuclear Research, Dubna;
%
National Research Foundation of Korea (NRF);
%
Consejo Nacional de Cienca y Tecnologia (CONACYT), Direccion General de Asuntos del Personal Academico(DGAPA), M\'{e}xico, Amerique Latine Formation academique - 
European Commission~(ALFA-EC) and the EPLANET Program~(European Particle Physics Latin American Network);
%
Stichting voor Fundamenteel Onderzoek der Materie (FOM) and the Nederlandse Organisatie voor Wetenschappelijk Onderzoek (NWO), Netherlands;
%
Research Council of Norway (NFR);
%
National Science Centre, Poland;
%
Ministry of National Education/Institute for Atomic Physics and National Council of Scientific Research in Higher Education~(CNCSI-UEFISCDI), Romania;
%
Ministry of Education and Science of Russian Federation, Russian
Academy of Sciences, Russian Federal Agency of Atomic Energy,
Russian Federal Agency for Science and Innovations and The Russian
Foundation for Basic Research;
%
Ministry of Education of Slovakia;
%
Department of Science and Technology, South Africa;
%
Centro de Investigaciones Energeticas, Medioambientales y Tecnologicas (CIEMAT), E-Infrastructure shared between Europe and Latin America (EELA), 
Ministerio de Econom\'{i}a y Competitividad (MINECO) of Spain, Xunta de Galicia (Conseller\'{\i}a de Educaci\'{o}n),
Centro de Aplicaciones Tecnológicas y Desarrollo Nuclear (CEA\-DEN), Cubaenerg\'{\i}a, Cuba, and IAEA (International Atomic Energy Agency);
%
Swedish Research Council (VR) and Knut $\&$ Alice Wallenberg
Foundation (KAW);
%
Ukraine Ministry of Education and Science;
%
United Kingdom Science and Technology Facilities Council (STFC);
%
The United States Department of Energy, the United States National
Science Foundation, the State of Texas, and the State of Ohio;
%
Ministry of Science, Education and Sports of Croatia and  Unity through Knowledge Fund, Croatia;
%
Council of Scientific and Industrial Research (CSIR), New Delhi, India;
%
Pontificia Universidad Cat\'{o}lica del Per\'{u}.


==> texs/notes.tex <==
%%
%% Notes for the IRC
%%
\section{Notes}

This appendix contains assorted notes for the ALICE collaborators, in
particular the PC, IRC, and EB. 

\begin{itemize}
\item Current length count is $\le 3\,600$ words. Of these
  $\approx3\,000$ are text and the remaining $600$ are from figures
  (with the model plot being $106$ words). The PRL limit is
  $3\,500$. 
\item The number of fits on \figref{fig:TotalNchSys_05023} could be
  cut down as it tends to clutter the plot, and not all of them are
  very informative. 
\item To-do items are 
  \begin{itemize}
  \item Get confirmation from Flemming on ``private communication''.
  \end{itemize}
\end{itemize}

%% Local Variables:
%%  TeX-master: "../cds"
%%  ispell-local-dictionary: "british"
%% End:

%  LocalWords:  Kolomogorov ndf pseudorapidity symmetrised SPD FMD
%  LocalWords:  pseudorapidities parametrisation Glauber PbPb LHC KLN
%  LocalWords:  Hijing EPOS pions kaons Jacobian Carruthers RHIC

